Rapid Quadrotor Navigation in Diverse Environments using an Onboard Depth Camera

Search and rescue environments exhibit challenging 3D geometry (e.g., confined spaces, rubble, and breakdown), which necessitates agile and maneuverable aerial robotic systems. Because these systems are size, weight, and power (SWaP) constrained, rapid navigation is essential for maximizing environment coverage. Onboard autonomy must be robust to prevent collisions, which may endanger rescuers and victims. Prior works have developed high-speed navigation solutions for autonomous aerial systems, but few have considered safety for search and rescue applications. These works have also not demonstrated their approaches in diverse environments. We bridge this gap in the state of the art by developing a reactive planner using forward-arc motion primitives, which leverages a history of RGB-D observations to safely maneuver in close proximity to obstacles. At every planning round, a safe stopping action is scheduled, which is executed if no feasible motion plan is found at the next planning round. The approach is evaluated in thousands of simulations and deployed in diverse environments, including caves and forests. The results demonstrate a 24% increase in success rate compared to state-of-the-art approaches.

==> content/contributions.tex <==
The contributions of this work are: (1) a reactive navigation
framework that uses a history of depth observations to evaluate a
library of forward-arc motion primitives; (2) a trajectory scheduling
approach to prevent collisions; (3) extensive photo-realistic
simulations with 3150 trials in diverse cluttered environments; and
(4) hardware experiments covering \SI{205}{\meter} collision-free with a
maximum speed of $\SI{6}{\meter\per\second}$.
The results demonstrate $24\%$ higher success compared to state of the
art approaches.

